Principled Ultrasound Data Augmentation for Classification of Standard Planes

Deep learning models with large learning capacities often overfit to medical imaging datasets. This is because training sets are often relatively small due to the significant time and financial costs incurred in medical data acquisition and labelling. Data augmentation is therefore often used to expand the availability of training data and to increase generalization. However, augmentation strategies are often chosen on an ad-hoc basis without justification. In this paper, we present an augmentation policy search method with the goal of improving model classification performance. We include in the augmentation policy search additional transformations that are often used in medical image analysis and evaluate their performance. In addition, we extend the augmentation policy search to include non-linear mixed-example data augmentation strategies. Using these learned policies, we show that principled data augmentation for medical image model training can lead to significant improvements in ultrasound standard plane detection, with an an average F1-score improvement of 7.0% overall over naive data augmentation strategies in ultrasound fetal standard plane classification. We find that the learned representations of ultrasound images are better clustered and defined with optimized data augmentation.

==> Backups/backupbib.tex <==
\begin{thebibliography}{}

\bibitem{RichardIPMI}
Droste, R, et al. “Ultrasound Image Representation Learning by Modeling Sonographer Visual Attention.” Information Processing in Medical Imaging, 2019.
\bibitem{SEResnet}
Hu, Jie, et al. “Squeeze-and-Excitation Networks.” in IEEE Transactions on Pattern Analysis and Machine Intelligence, 2020.
\bibitem{luke}
Luke T, Geoff N, "Improving deep learning using generic data augmentation," in IEEE Symposium Series on Computational Intelligence, 2018.
\bibitem{ce}
Cecilia S, Michael JD, "Improved mixed-example data augmentation," in IEEE Winter Conference on Applications of Computer Vision (WACV), 2019. 
\bibitem{ryo}
Ryo T, Takashi M, "Data augmentation using random image cropping and patches for deep CNNs," in IEEE Transactions on Circuits and Systems for Video Technology, 2020. 
\bibitem{gz}
Gan Z, Henao R, Carlson D, Carin L, "Learning deep sigmoid belief networks with data augmentation," in Proceedings of Machine Learning Research (PMLR), 2015. 
\bibitem{ho}
Hiroshi Ohno." Auto-encoder-based generative models for data augmentation on regression problems," in Soft Computing, 2019. 
\bibitem{ze}
Z. Eaton-Rosen, F. Bragman, S. Ourselin, and M. J. Cardoso, "Improving data augmentation for medical image segmentation," in International Conference on Medical Imaging with Deep Learning (MIDL), 2018.
\bibitem{mf}
M. Frid-Adar, I. Diamant, E. Klang, M. Amitai, J. Goldberger, and H. Greenspan, "GAN-based synthetic medical image augmentation for increased CNN performance in liver lesion classification," in Neurocomputing, vol. 321, pp. 321–331, Dec. 2018.
\bibitem{dj}
D. Jin, Z. Xu, Y. Tang, A. P. Harrison, and D. J. Mollura, "CT-realistic lung nodule simulation from 3D conditional generative adversarial networks for robust lung segmentation," in MICCAI, 2018.
\bibitem{zab}
Zhao, A., Balakrishnan, G., Durand, F., Guttag, J.V., Dalca, A.V., "Data augmentation using learned transformations for one-shot medical image segmentation," in CVPR, 2019, pp. 8543–8553.
\bibitem{df}
Dubost F, Bortsova G, Adams H, Ikram M.A., Niessen W, Vernooij M and De Bruijne M, "Hydranet: Data Augmentation for Regression Neural Networks," in MICCAI, 2019. 
\bibitem{azhp}
Asaduz Z, Sang H.P., Hyunhee B, Chul-woo P, Ilhyung P and Sanghyun J, "Generative approach for data augmentation for deep learning-based bone surface segmentation from ultrasound images," in International Journal of Computer Assisted Radiology and Surgery volume 15, 2020, pages931–941.
\bibitem{ghl}
C. Han, L. Rundo, R. Araki, Y. Furukawa, G. Mauri, H. Nakayama, and H. Hayashi, "Infinite brain MR images: PGGAN-based data augmentation for tumor detection," in Neural Approaches to Dynamics of Signal Exchanges(Smart Innovation, Systems and Technologies), 2019, pp. 291–303.
\bibitem{mam}
Mikoajczyk, A, and Grochowski, M, "Data augmentation for improving deep learning in image classification problem," in Proceedings International Interdisciplinary PhD Workshop (IIPhDW), 2018, pp. 117–122.
\bibitem{zhf}
Z. Hussain, F. Gimenez, D. Yi, and D. Rubin, "Differential data augmentation techniques for medical imaging classification tasks," in AMIA Annual Symposium Proceedings, volume 2017, page 979. 
\bibitem{hzmc}
H. Zhang, M. Cisse, Y. N. Dauphin, and D. Lopez-Paz ,"mixup: Beyond empirical risk minimization," in International Conference on Learning Representations (ICLR), 2018. 
\bibitem{aoc}
Augustus O, Christopher O, and Jonathon S, "Conditional image synthesis with auxiliary classifier GANs," in International Conference on Learning Representations (ICLR), 2017.
\bibitem{pgone}
Karras, T., Aila, T., Laine, S., and Lehtinen, J, "Progressive growing of GANs for improved quality, stability, and variation," in International Conference on Learning Representations (ICLR), 2018.
\bibitem{edcb}
E. D. Cubuk, B. Zoph, D. Mane, V. Vasudevan, and Q. V. Le, ‘‘AutoAugment: Learning augmentation strategies from data,’’ in International Conference on Computer Vision Pattern Recognition (CVPR), 2019.
\bibitem{dhel}
D. Ho, E. Liang, X. Chen, I. Stoica, and P. Abbeel, “Population Based Augmentation: Efficient Learning of Augmentation Policy Schedules,” in International Conference on Machine Learning (ICML), 2019.
\bibitem{slik}
S. Lim, I. Kim, T. Kim, C. Kim, and S. Kim, "Fast autoaugment," in Advances in Neural Information
Processing Systems (NeurIPs), pages 6662–6672, 2019.
\bibitem{CMJ}
C. Summers and M.J Dinneen, "Improved mixed example data augmentation," in IEEE Winter Conference on Applications of Computer Vision (WACV), 2019.
\bibitem{tyy}
Tokozume, Y., Ushiku, Y., and Harada, T, "Between-class learning for image classification," in The IEEE Conference on Computer Vision and Pattern Recognition (CVPR), 2018.
\bibitem{ebj}
E. D. Cubuk, B. Zoph, J. Shlens, and Q. V. Le, "Randaugment: Practical automated data augmentation with a reduced search space," in The IEEE Conference on Computer Vision and Pattern Recognition (CVPR), 2020.
\bibitem{avi}
A. Buslaev1, V.I. Iglovikov, E. Khvedchenya, A. Parinov ,M. Druzhinin and A. A. Kalinin, "Albumentations: Fast and Flexible Image Augmentations, " in MDPI Journal of Information, 2020.
\bibitem{blsa}
Bargsten, L., Schlaefer, A, "SpeckleGAN: a generative adversarial network with an adaptive speckle layer to augment limited training data for ultrasound image processing, " in Int J CARS 15, 1427–1436 (2020).
\bibitem{rsjj}
R. Gontijo-Lopes, S. J. Smullin, E. D. Cubuk, and E. Dyer. Affinity and diversity: Quantifying mechanisms of data augmentation. arXiv preprint arXiv:2002.08973, 2020
\bibitem{nal}
J. Nalepa et al., "Data Augmentation via Image Registration," IEEE International Conference on Image Processing (ICIP), 2019
\bibitem{mixaug}
C. Summers and M. J. Dinneen, "Improved Mixed-Example Data Augmentation," IEEE Winter Conference on Applications of Computer Vision (WACV), 2019
\bibitem{Sononet}
C. F. Baumgartner et al., "SonoNet: Real-Time Detection and Localisation of Fetal Standard Scan Planes in Freehand Ultrasound," in IEEE Transactions on Medical Imaging, 2017
\bibitem{jbi}
Jiao, J., et al. “Self-Supervised Representation Learning for Ultrasound Video.” 2020 IEEE 17th International Symposium on Biomedical Imaging, 2020

\end{thebibliography}
